Neural Free-Viewpoint Relighting for Glossy Indirect Illumination

Precomputed Radiance Transfer (PRT) remains an attractive solution for real-time rendering of complex light transport effects such as glossy global illumination. After precomputation, we can relight the scene with new environment maps while changing viewpoint in real-time. However, practical PRT methods are usually limited to low-frequency spherical harmonic lighting. All-frequency techniques using wavelets are promising but have so far had little practical impact. The curse of dimensionality and much higher data requirements have typically limited them to relighting with fixed view or only direct lighting with triple product integrals. In this paper, we demonstrate a hybrid neural-wavelet PRT solution to high-frequency indirect illumination, including glossy reflection, for relighting with changing view. Specifically, we seek to represent the light transport function in the Haar wavelet basis. For global illumination, we learn the wavelet transport using a small multi-layer perceptron (MLP) applied to a feature field as a function of spatial location and wavelet index, with reflected direction and material parameters being other MLP inputs. We optimize/learn the feature field (compactly represented by a tensor decomposition) and MLP parameters from multiple images of the scene under different lighting and viewing conditions. We demonstrate real-time (512 x 512 at 24 FPS, 800 x 600 at 13 FPS) precomputed rendering of challenging scenes involving view-dependent reflections and even caustics.

==> paper_body/algorithm.tex <==
\section{Algorithm}


\begin{table*}[h]
    \centering
    \begin{tabular}{l|l}
    Variable & Definition \\ \hline
    $X$ & scene \\
    $x$ & vertex $\in [0, 1]^3$ of 3D surface \\
    $\xi$ & wavelet value \\
    $n_x$ & normal at $x$ \\
    $T^{\text{indirect}}(x, \omega, \omega_o)$ & $[0, 1]^3 \times \mathbb{S}^2 \times \mathbb{S}^2 \rightarrow \mathbb{R}^3$. Indirect light transport operator. Represents 6D surface indirect light field. \\
    $\mathbf{T}(\omega_o)$ & discretized $\omega_o$-slice of $T$ tensor. rows represent $x$, cols represent $\xi$ \\
    $i$ & index of particular row of $\mathbf{T}$, or how a scene point scatters $n$ wavelet lights \\
    $j$ & index of particular col of $\mathbf{T}$, or how all scene points scatter a wavelet light \\
    $\omega_r$ & $\omega_o - 2(\omega_o \cdot n_x)n_x$ \\
    $\mathbf{L}$ & Environment map \\
    $n$ & Size of the environment map \\ \hline
    $W$ & 2D orthogonal wavelet transform operation \\
    $\{\Psi_k\}\limits_{k=1}^{n}$ & discrete 2D wavelet basis functions \\
    $h(x, j)$ & $[0, 1]^2 \times \mathbb{R}^{n} \rightarrow \mathbb{R}^P$;  $P$-dim feature vector $d$ to be decoded \\ 
    $R_{fg}$ & spatial feature grid size \\
    $R$ & rank of expansion \\
    $P$ & feature dim \\
    $H$ & $\in \mathbb{R}^{R_{fg} \times n \times P}$; discrete feature grid that will approximate continuous $h$ \\
    $\mathrm{MLP}(h(x, j), \omega_r, k_d, k_s, \rho)$ & $\mathbb{R}^P \times \mathbb{S}^2 \times \cdots \rightarrow \mathrm{2D\,\,wavelets}$; Transport coefficient $\mathbf{T}(\omega_o)_{ij}$ \\ \hline
    $p_x \times p_y$ & dimensions of image \\
    $g(X, \mathbf{L}, \omega_o, k_d, k_s, \rho)$ & $[0, 1]^2 \times \mathbb{R}^n \times \mathbb{S}^2 \times \cdots \rightarrow \mathbb{R}^{p_x \times p_y}$; 128spp denoising path tracer \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}

\begin{figure*}[t]
\centering
   \includegraphics[width=\linewidth]{paper_body/figures/pipeline.png}
\caption{\em \textbf{I am a placeholder} Overview of our pipeline.}
\label{fig:pipeline}
\end{figure*}


\subsection{Multi-Bounce Light Transport}
We want to construct the definition of the multi-bounce light transport operator. For a scene lit only by emission in the far-field, such that the incoming radiance is only a function of angle, the rendering equation that describes the scattered radiance from a point $x$ on the scene manifold towards the direction $\omega_o$ is as follows:

\begin{equation}
    L_o(x, \omega_o) = \int\limits_{\Omega} L_i(\omega_i) f(x, \omega, \omega_o) V(x, \omega) (n \cdot \omega) d\omega
\end{equation}
where $f(x, \omega, \omega_o)$ is the bidirectional reflectance distribution function and $V(x, \omega)$ is the visibility operator. Following the derivation of [Wang, et al. 2006] [TODO: add citations], we describe the \textit{outgoing radiance} of the first bounce $L_o^1(x, \omega_o)$ from a point $x$ along direction $\omega_o$ as follows: 
    
\begin{equation}
    L_o^1(x, \omega_o) = \int\limits_{\Omega} L_o(\tilde{x}(x, \omega), -\omega) f(x, \omega, \omega_o) (1 - V(x, \omega)) (n \cdot \omega) d\omega
\end{equation}
where $\tilde{x}(x, \omega)$ is the first point on the scene manifold that $x$ observes in direction $\omega$. Equation 2 simply states that the outgoing radiance from point $x$ to all seen points $\tilde{x}$ is attenuated by the BRDF. Let $T(x, \omega, \omega_o) = f(x, \omega, \omega_o)V(x,\omega)(n\cdot\omega)$ be called the \textit{transport operator} and let $\widebar{T}(x, \omega, \omega_o) = f(x, \omega, \omega_o)(1-V(x,\omega))(n\cdot\omega)$ be called the \textit{complementary transport operator}. Define $\tilde{x}\,\,\dot=\,\,\tilde{x}(x, \omega)$ for simplicity. Recursively substituting Equation 1 in Equation 2 produces:

\begin{align}
    L_o^1(x, \omega_o) &= \int\limits_{\Omega} \int\limits_{\Omega} L(\omega) T(\tilde{x}, \omega, -\omega') \widebar{T}(x, \omega', \omega_o) d\omega' d\omega \\
    &= \int\limits_{\Omega} L(\omega) \left( \int\limits_{\Omega} T(\tilde{x}, \omega, -\omega') \widebar{T}(x, \omega', \omega_o) d\omega' \right) d\omega
\end{align}

Let the inner quantity be defined as the \textit{bounced transport operator} $T^1(x, \omega, \omega_o)$, representing the quantity of light bounced from all points $\tilde{x}$ via their respective transport functions $T$ attenuated by the complementary transport operator evaluated at $x$. As in [Wang, et al. 2006], bounced transport operators at higher bounces $n$ (representing indirect illumination) can be evaluated by further recursive substitution:

\begin{equation}
    T^n(x, \omega, \omega_o) &= \int\limits_{\Omega} T^{n-1}(\tilde{x}, \omega, -\omega') \widebar{T}(x, \omega', \omega_o) d\omega'
\end{equation}
where $T^0 \,\,\dot=\,\, T$. Due to the linearity of light transport, both the scattered radiance along $\omega_o$ and the bounced transport operators are additive along all bounces:

\begin{align}
    L_o^{\infty}(x, \omega_o) &= L_o(x, \omega_o) + L_o^1(x, \omega_o) + \cdots \\
    T^\infty(x, \omega, \omega_o) &= T(x, \omega, \omega_o) + T^1(x, \omega, \omega_o) + \cdots 
\end{align}

where the first terms in each represent direct illumination, and the rest of the terms represent indirect illumination:

\begin{align}
    L_o^{\text{indirect}}(x, \omega_o) &= \sum_{i=1}^{\infty} L_o^i(x, \omega_o) \\
    T^{\text{indirect}}(x, \omega, \omega_o) &= \sum_{i=1}^{\infty} T^i(x, \omega, \omega_o) 
\end{align}

Many formulations exist in real-time ray tracing and precomputed radiance transfer to represent the direct illumination $L_o$ via the direct transport operator $T$, such as [Triple Product Wavelet Integrals]. However, there are no formulations in classical precomputed radiance transfer that are able to represent arbitrary global illumination via the all-frequency indirect transport operator for any viewpoint. This is because $T^{\text{indirect}}$ is a dense six-dimensional function that is prohibitively large in storage. However, recent advances in neural implicit function representation have demonstrably availed this problem, allowing the regression of $T^{\text{indirect}}$ given samples of $L_o^{\text{indirect}}$.
    
\subsection{Wavelet Basis Representation}
We aim to globally learn the entire six-dimensional surface indirect-light field of a synthetic scene $X$. However, even for neural regression, properly sampling this dense function would pose significant problems and previous methods aiming to render a scene could do so from a novel view or novel lighting, but not both. We aim to solve both problems at once by performing both the regression and rendering in the wavelet domain. If, for a fixed $\omega_o$, the discrete transport operator $\mathbf{T}(\omega_o)$ is represented in an orthogonal 2D discrete wavelet basis $\{\Psi_k\}_{k=1}^{n}$ then the all-frequency double product integral reduces to a simple dot product:

\begin{align}
    L_o^{\text{indir}}(x, \omega_o) &= \int\limits_{\mathbb{S}^2} \left(\sum_{j=1}^{n} \mathbf{T}(x,\omega_o)_{ij} \Psi_j(\omega)\right) \left(\sum_{k=1}^{n} \mathbf{L}_k \Psi_k(\omega)\right) d\omega \\
    &= \sum_j \sum_k \mathbf{T}(x,\omega_o)_{ij} \mathbf{L}_k \braket{\Psi_j|\Psi_k} = \mathbf{T}(x,\omega_o)_i \cdot \mathbf{L}
\end{align}
with the integral over the whole sphere, and $T(x,\omega_o)$ is set to 0 in the lower hemisphere. 

Regression directly in the wavelet basis has several advantages. It is well-established that the discrete transport operators are sparse in the wavelet domain, as most of the frequencies are concentrated in relatively few entries. This makes the problem of memorizing the surface light field for a particular scene tractable. Second, we can compute the all-frequency rendering equation directly, avoiding the need for low-frequency approximations or using neural networks as renderers. This makes our method agnostic to both view and lighting, enabling full generalization for complex light transport effects. Zoinks! 

\subsection{Method Overview}

We aim to solve the following optimization function
\begin{equation}
    \underset{f}{\mathrm{arg\,\,min} } \,\, \left\Vert \ell\left( \sum_{j=1}^{n}\mathrm{MLP}(h(x, j), \omega_r, n_x, k_d, k_s, \rho)W\{\mathbf{L}\}, g(x, \mathbf{L}, \omega_o, k_d, k_s, \rho)\right) \right\Vert_2^2
\end{equation}
where $\ell$ is a modified $L^2$-loss function. $\text{MLP}$ is a very small multilayer perceptron that decodes a feature field into wavelet coefficients for each scene point on the screen. $h$ represents a feature field indexed by the surface point $x$ and a particular wavelet index $j$. This feature field aims to capture how a wavelet light at index $j$ scatters when encountering a scene point $x$, and so a particular sampling of this feature field returns a feature vector that describes this. The additional information passed to the MLP aims to provide additional information how how this scattered light is reflected towards the viewing direction. We want to keep all computations in the wavelet domain. Consider the function $h(x, j)$ of the spatial coordinate and the wavelet index, which attempts to measure how much the light from a wavelet light $\xi$ scatters as soon as it hits a particular scene point $x$. 

\subsubsection{Design of the Neural Spatio-Wavelet Light Function}

We will represent the full continuous spatio-wavelet light function $h$ as an $R_{fg} \times n \times P$ feature tensor $H$. Let $a, b, c$ represent the discrete indices of the feature tensor along the three axes (spatial, wavelet and feature, respectively), so that indexing $H_{abc}$ refers to a single element, and $H_{ab}$ refers to a $P$-dimensional vector describing how the wavelet at $b$ interacts with the point at $a$. Let us perform a rank-$R$ decomposition of this tensor, representing it as a sum of $R$ low-rank feature tensors:

\begin{equation}
    H = \sum_{r=1}^{R} \mathcal{A}_{r}
\end{equation}

We now have a set of $R$ feature tensors $\mathcal{A}_r$ of size $R_{fg} \times n \times P$. Now, we perform CP decomposition of these tensors along the three modes: a spatial location vector $\mathcal{A}_{r}^{\mathrm{spatial}} \in \mathbb{R}^{R_{fg} \times R}$, wavelet location vector $\mathcal{A}_{r}^{\mathrm{wavelet}} \in \mathbb{R}^{n \times R}$, and the feature vector $b_r^{\text{feature}}$, which is of much lower rank than the spatial and wavelet dimensions:

\begin{equation}
    H = \sum_{r=1}^{R} \mathcal{A}_{r}^{\mathrm{spatial}} \otimes \mathcal{A}_{r}^{\mathrm{wavelet}} \otimes b_r^{\mathrm{feature}}
\end{equation}
where $\otimes$ represents an outer product along a new dimension. 

We represent $\mathcal{A}_{r}^{\mathrm{spatial}}$ as a three-dimensional multiresolution hash encodings [InstantNGP]. We perform trilinear interpolation on the feature grid to produce a feature vector of length $R$. Though ideally one would store a different feature vector for each wavelet, for consistency we also represent $\mathcal{A}_{r}^{\mathrm{wavelet}}$ as a two-dimensional multiresolution feature grid to produce a feature vector of length $R$. We try to minimize the spatial locality as much as possible in the wavelet grid as there does not need to be spatial locality in the wavelet domain. The feature vector $b_r$ is represented as an $R \times P$ learnable matrix, equivalent to a single neural network layer without bias. Then, we estimate the value of $h(x, j)$ as 

\begin{equation}
    h(x, j) = B \left(\mathcal{A}^{\mathrm{spatial}}(x) \odot \mathcal{A}^{\mathrm{wavelet}}(j)\right) \in \mathbb{R}^P 
\end{equation}
where $\odot$ is a pointwise multiplication.

\subsubsection{Design of the Neural Network}

\begin{table}[]
    \centering
    \begin{tabular}{c c c} \hline
        Parameter & Symbol & Encoding \\ \hline
        Wavelet-scattered feature vector & $h(x, j)$ & $\mathrm{Id}(h(x,j)) \in \mathbb{R}^{64}$ \\ \hline
        Reflection dir. & $\omega_r$ & $ \mathrm{OB}(\omega_r) \in \mathbb{R}^{3\times 4}$ \\ \hline 
        Normal & $n_x$ & $\mathrm{OB}(n_x) \in \mathbb{R}^{3\times 4}$ \\ \hline 
        Roughness & $\rho$ & $ \mathrm{OB}\left(\frac{\mathrm{log}(25x+1)}{\mathrm{log}(25+1)}\right) \in \mathbb{R}^{1\times 4}$ \\ \hline 
        Specular albedo & $k_s$ & $\mathrm{Id}(k_s) \in \mathbb{R}^{3\times 1}$ \\ \hline
        Diffuse albedo & $k_d$ & $\mathrm{Id}(k_d) \in \mathbb{R}^{3\times 1}$ \\ \hline
    \end{tabular}
    \caption{Encodings of Inputs to the Decoder MLP}
    \label{tab:encodings}
\end{table}
We use a shallow MLP to decode the feature vector $h(x, j)$ with additional information from the geometry buffer at the scene point $x$. We encode much of this additional information with the one-blob encoding from [Neural Radiance Cache] with $k=4$ bins. The exact encodings can be found in Table \ref{tab:encodings}. This network outputs a single dual wavelet coefficient for the point $x$ and wavelet index $j$, which can be visualized as a single element of the indirect light transport operator in wavelet space. Evaluating this network for a single scene point $x$ and all the wavelet indices $j$ of the environment map produces a row of this tensor, and evaluating it for all scene points $x$ and a single wavelet index $j$ produces a column of this tensor. Since the regression is done directly in the wavelet basis, the rendering equation can be computed by directly multiplying the output of the MLP with the wavelet-transformed environment map, producing all-frequency light transport effects. 
